Easy High-Dimensional Likelihood-Free Inference

We introduce a framework using Generative Adversarial Networks (GANs) for likelihood--free inference (LFI) and Approximate Bayesian Computation (ABC) where we replace the black-box simulator model with an approximator network and generate a rich set of summary features in a data driven fashion. On benchmark data sets, our approach improves on others with respect to scalability, ability to handle high dimensional data and complex probability distributions.

==> gan-tikz.tex <==
\begin{tikzpicture}[auto,
block/.style={rectangle, thick,draw=blue!80,rounded corners},
cmath/.style={rectangle},
mmd/.style={circle,draw=red!80},
branch/.style={fill,shape=circle,minimum size=3pt,inner sep=0pt},
line/.style ={->,draw, thick, -latex', shorten >=0pt}]
\matrix[column sep=1.5cm,row sep=1cm]{ 
 &  \node (D) [block] {Discriminator};
& \node (D') [mmd] {MMD}; \\
\node (O) [cmath] {${\cal O}$ (observed)}; 
& \node (S') [block] {Approx. Simulator $S'$};
& \node (S) [block] {simulator $S$}; \\
  & 
\node (G) [block] {Generator}; \\
 & \node (prior_theta) [cmath] {$q_{\theta}(\theta)$ (prior)};
 & \node (noise) [cmath] {$\omega$ (noise)}; \\
};
\begin{scope}[every path/.style=line]
\path (prior_theta) --   (G); 
\path (noise) -- (S); 
\path (noise) -- coordinate (branch)  (S'); 
\path (G) -- (S);
\path (G) -- (S');
\path (S') -- (D');
\path (S') -- (D);
\path (S) -- (D'); 
\path (O) -- (D);
\end{scope}
\end{tikzpicture}

==> mmd-gan-tikz.tex <==
\begin{tikzpicture}[auto,
block/.style={rectangle, thick,draw=blue!80,rounded corners},
cmath/.style={rectangle},
mmd/.style={circle,draw=red!80},
branch/.style={fill,shape=circle,minimum size=3pt,inner sep=0pt},
line/.style ={->,draw, thick, -latex', shorten >=0pt}]
\matrix[column sep=1.5cm,row sep=1cm]{ 
\node (D) [mmd] {MMD}; &  
& \node (D') [mmd] {MMD}; \\
\node (O) [cmath] {${\cal O}$ (observed)}; 
& \node (S') [block] {Approx. Simulator $S'$};
& \node (S) [block] {simulator $S$}; \\
  & 
\node (G) [block] {Generator}; \\
 & \node (prior_theta) [cmath] {$q_{\theta}(\theta)$ (prior)};
 & \node (noise) [cmath] {$\omega$ (noise)}; \\
};
\begin{scope}[every path/.style=line]
\path (prior_theta) --   (G); 
\path (noise) -- (S); 
\path (noise) -- coordinate (branch)  (S'); 
\path (G) -- (S);
\path (G) -- (S');
\path (S') -- (D');
\path (S') -- (D);
\path (S) -- (D'); 
\path (O) -- (D);
\end{scope}
\end{tikzpicture}
